Neural Token Segmentation for High Token-Internal Complexity

Tokenizing raw texts into word units is an essential pre-processing step for critical tasks in the NLP pipeline such as tagging, parsing, named entity recognition, and more. For most languages, this tokenization step straightforward. However, for languages with high token-internal complexity, further token-to-word segmentation is required. Previous canonical segmentation studies were based on character-level frameworks, with no contextualised representation involved. Contextualized vectors a la BERT show remarkable results in many applications, but were not shown to improve performance on linguistic segmentation per se. Here we propose a novel neural segmentation model which combines the best of both worlds, contextualised token representation and char-level decoding, which is particularly effective for languages with high token-internal complexity and extreme morphological ambiguity. Our model shows substantial improvements in segmentation accuracy on Hebrew and Arabic compared to the state-of-the-art, and leads to further improvements on downstream tasks such as Part-of-Speech Tagging, Dependency Parsing and Named-Entity Recognition, over existing pipelines. When comparing our segmentation-first pipeline with joint segmentation and labeling in the same settings, we show that, contrary to pre-neural studies, the pipeline performance is superior.

==> 2-related_works.tex <==
Few studies in the past addressed a multi-language segmentation model.
 
 UDPipe \cite{udpipe:2017} framework aims to create a simple-to-use model tool, to easily process raw text intto CoNLL-U-formatted data. UDPipe's focus was not on MRLs, but on a general model that will preform best on 90 languages in UD 2.5. It's tokenization model (which hasn't changed in UDPipe 2.0 \cite{straka-2018-udpipe}) is based on a bidirectional GRU \cite{cho2014learning}, and it's architecture intended to split tokens and sentences, not syntactic words. The paper even acknowledges that the tokenizer does not handle multi-word tokens. 

 Universal Word Segmentation \cite{DBLP:journals/corr/abs-1807-02974} prsented a universal character tagging model that preformed word segmentation. While this framework did show a significant increase on segmentation accuracies, The results on MRLs remained lagging far behind. The paper main focus was on using only the surface characters while morphological fusion creates forms that are implicit in the surface representation yet have to be recovered. 

 Lastly, PtrNetMD \cite{seker-tsarfaty-2020-pointer} is an end-to-end neural solution for both segmentation and POS tagging. It relies on first preforming morphological analysis(MA) on each word: extracting all the possible options for morphemes and their POS tags. Then, it uses a pointer network \cite{vinyals2017pointer} to chose the best option for the entire sentence. This model preformed reasonably well, achieving a new Hebrew SOTA result of 96.36\%, under the unrealistic assumption that the MA has complete lexical coverage. But The paper shows meaningful decrease in performance when no such MA is of presence, with accuracy of 94.74\%, compared to our 96.31\%. This framework relies heavily on providing a good MA solution, which is not easy to obtain on all languages, and is not provided as part of the UD project.

==> 2-the_challange.tex <==
In Languages like Hebrew or Arabic, basic `words' compose to form  tokens that consists of multiple meaning-bearing units. E.g., the  token   \textbf{\textit{\cjRL{wmhbyt}}} in Hebrew consists of four units with four distinct POS tags (\cjRL{w}-and (CONJ) + \cjRL{m}-from (ADP) + \cjRL{h}-the (DET) + \cjRL{byt}-house (NN)). However, the token composition is often not transparent in the character sequence of the token, which 
 leads to extreme token-internal ambiguity.  %
Consider, for example, the Hebrew token \textbf{\textit{\cjRL{b.slm}}}. It could map to: \cjRL{b--.sl--/sl--hm} (literally: in-shadow-of-them, meaning: in their shadow), \cjRL{b.sl--/sl--hm} (literally: onion-of-them, meaning: their onion), \cjRL{b--h--.slm} (literally: in-the-image, meaning: in the image) and  more. A-priory all analyses are equally likely. Only {\em in-context} the correct segmentation becomes available.

Accurate segmentation of tokens to words in these languages is critical, and  errors in segmentation lead to error propagation that severely contaminates the downstream task \cite{bareket2020neural, marton2010improving, green2010better}. %
In recent years, various language-specific neural segmentation models have been introduced.  %
 however, such models often make the unrealistic assumption that they have a full-coverage morphological analyzer at their disposal
 \cite{seker-tsarfaty-2020-pointer, zalmout2017don}.
An orthogonal line of works aims at  {\em language-agnostic} segmentation models that could be trained end-to-end given a gold (pre-segmented) corpus in any given language.
 UDPipe \cite{udpipe:2017} delivers such a universal segmenter    %
 that is based on character-labeling. However, this model does not attend to implicit forms, and  \newcite{udpipe:2017} acknowledge that  it does not handle multi-word tokens particularly well.
 A more recent work on Universal Word Segmentation (UAS) \cite{DBLP:journals/corr/abs-1807-02974} presented a universal character-tagging model that preformed substantially better than UDPipe on many languages. %
 But for languages with rich and ambiguous token compositions, the results still lag  behind. This work aims to remedy this situation, and offer a language-agnostic model that can be easily applied cross-linguistically yet is nonetheless effective in segmenting complex and highly ambigous tokens.

 


==> 7-acknowledgments.tex <==
We would like to thank Bar-Ilan-University NLP lab for the comments, advice and computational resources.
